Towards Natural Language-Driven Assembly Using Foundation Models

Large Language Models (LLMs) and strong vision models have enabled rapid research and development in the field of Vision-Language-Action models that enable robotic control. The main objective of these methods is to develop a generalist policy that can control robots with various embodiments. However, in industrial robotic applications such as automated assembly and disassembly, some tasks, such as insertion, demand greater accuracy and involve intricate factors like contact engagement, friction handling, and refined motor skills. Implementing these skills using a generalist policy is challenging because these policies might integrate further sensory data, including force or torque measurements, for enhanced precision. In our method, we present a global control policy based on LLMs that can transfer the control policy to a finite set of skills that are specifically trained to perform high-precision tasks through dynamic context switching. The integration of LLMs into this framework underscores their significance in not only interpreting and processing language inputs but also in enriching the control mechanisms for diverse and intricate robotic operations.

==> Bosch_IR/qqq.tex <==
This is pdfTeX, Version 3.14159265-2.6-1.40.18 (MiKTeX 2.9.6400 64-bit) (preloaded format=pdflatex 2021.3.7)  15 MAR 2021 16:44
entering extended mode
**./Sim2RealICML2021_IR.tex
(Sim2RealICML2021_IR.tex
LaTeX2e <2017-04-15>
Babel <3.12> and hyphenation patterns for 76 language(s) loaded.
("C:\Program Files\MiKTeX 2.9\tex\latex\koma-script\scrartcl.cls"
Document Class: scrartcl 2017/04/13 v3.23 KOMA-Script document class (article)
("C:\Program Files\MiKTeX 2.9\tex\latex\koma-script\scrkbase.sty"
Package: scrkbase 2017/04/13 v3.23 KOMA-Script package (KOMA-Script-dependent b
asics and keyval usage)

("C:\Program Files\MiKTeX 2.9\tex\latex\koma-script\scrbase.sty"
Package: scrbase 2017/04/13 v3.23 KOMA-Script package (KOMA-Script-independent 
basics and keyval usage)

("C:\Program Files\MiKTeX 2.9\tex\latex\graphics\keyval.sty"
Package: keyval 2014/10/28 v1.15 key=value parser (DPC)
\KV@toks@=\toks14
)
("C:\Program Files\MiKTeX 2.9\tex\latex\koma-script\scrlfile.sty"
Package: scrlfile 2017/04/13 v3.23 KOMA-Script package (loading files)

Package scrlfile, 2017/04/13 v3.23 KOMA-Script package (loading files)
                  Copyright (C) Markus Kohm

))) ("C:\Program Files\MiKTeX 2.9\tex\latex\koma-script\tocbasic.sty"
Package: tocbasic 2017/04/13 v3.23 KOMA-Script package (handling toc-files)
\scr@dte@tocline@numberwidth=\skip41
\scr@dte@tocline@numbox=\box26
)
Package tocbasic Info: omitting babel extension for `toc'
(tocbasic)             because of feature `nobabel' available
(tocbasic)             for `toc' on input line 131.
Package tocbasic Info: omitting babel extension for `lof'
(tocbasic)             because of feature `nobabel' available
(tocbasic)             for `lof' on input line 133.
Package tocbasic Info: omitting babel extension for `lot'
(tocbasic)             because of feature `nobabel' available
(tocbasic)             for `lot' on input line 134.
Package scrartcl Info: You've used standard option `11pt'.
(scrartcl)             This is correct!
(scrartcl)             Internally I'm using `fontsize=11pt'.
(scrartcl)             If you'd like to set the option with \KOMAoptions,
(scrartcl)             you'd have to use `fontsize=11pt' there
(scrartcl)             instead of `11pt', too.
Class scrartcl Info: File `scrsize11pt.clo' used to setup font sizes on input l
ine 2059.

("C:\Program Files\MiKTeX 2.9\tex\latex\koma-script\scrsize11pt.clo"
File: scrsize11pt.clo 2017/04/13 v3.23 KOMA-Script font size class option (11pt
)
)
("C:\Program Files\MiKTeX 2.9\tex\latex\koma-script\typearea.sty"
Package: typearea 2017/04/13 v3.23 KOMA-Script package (type area)
\ta@bcor=\skip42
\ta@div=\count79
\ta@hblk=\skip43
\ta@vblk=\skip44
\ta@temp=\skip45
\footheight=\skip46
Package typearea Info: These are the values describing the layout:
(typearea)             DIV  = 10
(typearea)             BCOR = 0.0pt
(typearea)             \paperwidth      = 597.50793pt
(typearea)              \textwidth      = 418.25555pt
(typearea)              DIV departure   = -6%
(typearea)              \evensidemargin = 17.3562pt
(typearea)              \oddsidemargin  = 17.3562pt
(typearea)             \paperheight     = 845.04694pt
(typearea)              \textheight     = 595.80026pt
(typearea)              \topmargin      = -25.16531pt
(typearea)              \headheight     = 17.0pt
(typearea)              \headsep        = 20.40001pt
(typearea)              \topskip        = 11.0pt
(typearea)              \footskip       = 47.6pt
(typearea)              \baselineskip   = 13.6pt
(typearea)              on input line 1647.
)
\c@part=\count80
\c@section=\count81
\c@subsection=\count82
\c@subsubsection=\count83
\c@paragraph=\count84
\c@subparagraph=\count85
\scr@dte@part@maxnumwidth=\skip47
\scr@dte@section@maxnumwidth=\skip48
\scr@dte@subsection@maxnumwidth=\skip49
\scr@dte@subsubsection@maxnumwidth=\skip50
\scr@dte@paragraph@maxnumwidth=\skip51
\scr@dte@subparagraph@maxnumwidth=\skip52
LaTeX Info: Redefining \textsubscript on input line 4094.
\abovecaptionskip=\skip53
\belowcaptionskip=\skip54
\c@pti@nb@sid@b@x=\box27
\c@figure=\count86
\c@table=\count87
Class scrartcl Info: Redefining `\numberline' on input line 5233.
\bibindent=\dimen102
)
("C:\Program Files\MiKTeX 2.9\tex\generic\babel\babel.sty"
Package: babel 2017/06/29 3.12 The Babel package

("C:\Program Files\MiKTeX 2.9\tex\generic\babel\switch.def"
File: switch.def 2017/06/29 3.12 Babel switching mechanism
)
*************************************
* Local config file bblopts.cfg used
*
("C:\Program Files\MiKTeX 2.9\tex\latex\arabi\bblopts.cfg"
File: bblopts.cfg 2005/09/08 v0.1 add Arabic and Farsi to "declared" options of
 babel
)
("C:\Program Files\MiKTeX 2.9\tex\latex\babel-english\english.ldf"
Language: english 2017/06/06 v3.3r English support from the babel system

("C:\Program Files\MiKTeX 2.9\tex\generic\babel\babel.def"
File: babel.def 2017/06/29 3.12 Babel common definitions

("C:\Program Files\MiKTeX 2.9\tex\generic\babel\switch.def"
File: switch.def 2017/06/29 3.12 Babel switching mechanism
)
\babel@savecnt=\count88
\U@D=\dimen103
)
\l@canadian = a dialect from \language\l@american 
\l@australian = a dialect from \language\l@british 
\l@newzealand = a dialect from \language\l@british 
))
("C:\Program Files\MiKTeX 2.9\tex\latex\base\fontenc.sty"
Package: fontenc 2017/04/05 v2.0i Standard LaTeX package

("C:\Program Files\MiKTeX 2.9\tex\latex\base\t1enc.def"
File: t1enc.def 2017/04/05 v2.0i Standard LaTeX file
LaTeX Font Info:    Redeclaring font encoding T1 on input line 48.
))
("C:\Program Files\MiKTeX 2.9\tex\latex\base\inputenc.sty"
Package: inputenc 2015/03/17 v1.2c Input encoding file
\inpenc@prehook=\toks15
\inpenc@posthook=\toks16

("C:\Program Files\MiKTeX 2.9\tex\latex\base\utf8.def"
File: utf8.def 2017/01/28 v1.1t UTF-8 support for inputenc
Now handling font encoding OML ...
... no UTF-8 mapping file for font encoding OML
Now handling font encoding T1 ...
... processing UTF-8 mapping file for font encoding T1

("C:\Program Files\MiKTeX 2.9\tex\latex\base\t1enc.dfu"
File: t1enc.dfu 2017/01/28 v1.1t UTF-8 support for inputenc
   defining Unicode char U+00A0 (decimal 160)
   defining Unicode char U+00A1 (decimal 161)
   defining Unicode char U+00A3 (decimal 163)
   defining Unicode char U+00AB (decimal 171)
   defining Unicode char U+00AD (decimal 173)
   defining Unicode char U+00BB (decimal 187)
   defining Unicode char U+00BF (decimal 191)
   defining Unicode char U+00C0 (decimal 192)
   defining Unicode char U+00C1 (decimal 193)
   defining Unicode char U+00C2 (decimal 194)
   defining Unicode char U+00C3 (decimal 195)
   defining Unicode char U+00C4 (decimal 196)
   defining Unicode char U+00C5 (decimal 197)
   defining Unicode char U+00C6 (decimal 198)
   defining Unicode char U+00C7 (decimal 199)
   defining Unicode char U+00C8 (decimal 200)
   defining Unicode char U+00C9 (decimal 201)
   defining Unicode char U+00CA (decimal 202)
   defining Unicode char U+00CB (decimal 203)
   defining Unicode char U+00CC (decimal 204)
   defining Unicode char U+00CD (decimal 205)
   defining Unicode char U+00CE (decimal 206)
   defining Unicode char U+00CF (decimal 207)
   defining Unicode char U+00D0 (decimal 208)
   defining Unicode char U+00D1 (decimal 209)
   defining Unicode char U+00D2 (decimal 210)
   defining Unicode char U+00D3 (decimal 211)
   defining Unicode char U+00D4 (decimal 212)
   defining Unicode char U+00D5 (decimal 213)
   defining Unicode char U+00D6 (decimal 214)
   defining Unicode char U+00D8 (decimal 216)
   defining Unicode char U+00D9 (decimal 217)
   defining Unicode char U+00DA (decimal 218)
   defining Unicode char U+00DB (decimal 219)
   defining Unicode char U+00DC (decimal 220)
   defining Unicode char U+00DD (decimal 221)
   defining Unicode char U+00DE (decimal 222)
   defining Unicode char U+00DF (decimal 223)
   defining Unicode char U+00E0 (decimal 224)
   defining Unicode char U+00E1 (decimal 225)
   defining Unicode char U+00E2 (decimal 226)
   defining Unicode char U+00E3 (decimal 227)
   defining Unicode char U+00E4 (decimal 228)
   defining Unicode char U+00E5 (decimal 229)
   defining Unicode char U+00E6 (decimal 230)
   defining Unicode char U+00E7 (decimal 231)
   defining Unicode char U+00E8 (decimal 232)
   defining Unicode char U+00E9 (decimal 233)
   defining Unicode char U+00EA (decimal 234)
   defining Unicode char U+00EB (decimal 235)
   defining Unicode char U+00EC (decimal 236)
   defining Unicode char U+00ED (decimal 237)
   defining Unicode char U+00EE (decimal 238)
   defining Unicode char U+00EF (decimal 239)
   defining Unicode char U+00F0 (decimal 240)
   defining Unicode char U+00F1 (decimal 241)
   defining Unicode char U+00F2 (decimal 242)
   defining Unicode char U+00F3 (decimal 243)
   defining Unicode char U+00F4 (decimal 244)
   defining Unicode char U+00F5 (decimal 245)
   defining Unicode char U+00F6 (decimal 246)
   defining Unicode char U+00F8 (decimal 248)
   defining Unicode char U+00F9 (decimal 249)
   defining Unicode char U+00FA (decimal 250)
   defining Unicode char U+00FB (decimal 251)
   defining Unicode char U+00FC (decimal 252)
   defining Unicode char U+00FD (decimal 253)
   defining Unicode char U+00FE (decimal 254)
   defining Unicode char U+00FF (decimal 255)
   defining Unicode char U+0100 (decimal 256)
   defining Unicode char U+0101 (decimal 257)
   defining Unicode char U+0102 (decimal 258)
   defining Unicode char U+0103 (decimal 259)
   defining Unicode char U+0104 (decimal 260)
   defining Unicode char U+0105 (decimal 261)
   defining Unicode char U+0106 (decimal 262)
   defining Unicode char U+0107 (decimal 263)
   defining Unicode char U+0108 (decimal 264)
   defining Unicode char U+0109 (decimal 265)
   defining Unicode char U+010A (decimal 266)
   defining Unicode char U+010B (decimal 267)
   defining Unicode char U+010C (decimal 268)
   defining Unicode char U+010D (decimal 269)
   defining Unicode char U+010E (decimal 270)
   defining Unicode char U+010F (decimal 271)
   defining Unicode char U+0110 (decimal 272)
   defining Unicode char U+0111 (decimal 273)
   defining Unicode char U+0112 (decimal 274)
   defining Unicode char U+0113 (decimal 275)
   defining Unicode char U+0114 (decimal 276)
   defining Unicode char U+0115 (decimal 277)
   defining Unicode char U+0116 (decimal 278)
   defining Unicode char U+0117 (decimal 279)
   defining Unicode char U+0118 (decimal 280)
   defining Unicode char U+0119 (decimal 281)
   defining Unicode char U+011A (decimal 282)
   defining Unicode char U+011B (decimal 283)
   defining Unicode char U+011C (decimal 284)
   defining Unicode char U+011D (decimal 285)
   defining Unicode char U+011E (decimal 286)
   defining Unicode char U+011F (decimal 287)
   defining Unicode char U+0120 (decimal 288)
   defining Unicode char U+0121 (decimal 289)
   defining Unicode char U+0122 (decimal 290)
   defining Unicode char U+0123 (decimal 291)
   defining Unicode char U+0124 (decimal 292)
   defining Unicode char U+0125 (decimal 293)
   defining Unicode char U+0128 (decimal 296)
   defining Unicode char U+0129 (decimal 297)
   defining Unicode char U+012A (decimal 298)
   defining Unicode char U+012B (decimal 299)
   defining Unicode char U+012C (decimal 300)
   defining Unicode char U+012D (decimal 301)
   defining Unicode char U+012E (decimal 302)
   defining Unicode char U+012F (decimal 303)
   defining Unicode char U+0130 (decimal 304)
   defining Unicode char U+0131 (decimal 305)
   defining Unicode char U+0132 (decimal 306)
   defining Unicode char U+0133 (decimal 307)
   defining Unicode char U+0134 (decimal 308)
   defining Unicode char U+0135 (decimal 309)
   defining Unicode char U+0136 (decimal 310)
   defining Unicode char U+0137 (decimal 311)
   defining Unicode char U+0139 (decimal 313)
   defining Unicode char U+013A (decimal 314)
   defining Unicode char U+013B (decimal 315)
   defining Unicode char U+013C (decimal 316)
   defining Unicode char U+013D (decimal 317)
   defining Unicode char U+013E (decimal 318)
   defining Unicode char U+0141 (decimal 321)
   defining Unicode char U+0142 (decimal 322)
   defining Unicode char U+0143 (decimal 323)
   defining Unicode char U+0144 (decimal 324)
   defining Unicode char U+0145 (decimal 325)
   defining Unicode char U+0146 (decimal 326)
   defining Unicode char U+0147 (decimal 327)
   defining Unicode char U+0148 (decimal 328)
   defining Unicode char U+014A (decimal 330)
   defining Unicode char U+014B (decimal 331)
   defining Unicode char U+014C (decimal 332)
   defining Unicode char U+014D (decimal 333)
   defining Unicode char U+014E (decimal 334)
   defining Unicode char U+014F (decimal 335)
   defining Unicode char U+0150 (decimal 336)
   defining Unicode char U+0151 (decimal 337)
   defining Unicode char U+0152 (decimal 338)
   defining Unicode char U+0153 (decimal 339)
   defining Unicode char U+0154 (decimal 340)
   defining Unicode char U+0155 (decimal 341)
   defining Unicode char U+0156 (decimal 342)
   defining Unicode char U+0157 (decimal 343)
   defining Unicode char U+0158 (decimal 344)
   defining Unicode char U+0159 (decimal 345)
   defining Unicode char U+015A (decimal 346)
   defining Unicode char U+015B (decimal 347)
   defining Unicode char U+015C (decimal 348)
   defining Unicode char U+015D (decimal 349)
   defining Unicode char U+015E (decimal 350)
   defining Unicode char U+015F (decimal 351)
   defining Unicode char U+0160 (decimal 352)
   defining Unicode char U+0161 (decimal 353)
   defining Unicode char U+0162 (decimal 354)
   defining Unicode char U+0163 (decimal 355)
   defining Unicode char U+0164 (decimal 356)
   defining Unicode char U+0165 (decimal 357)
   defining Unicode char U+0168 (decimal 360)
   defining Unicode char U+0169 (decimal 361)
   defining Unicode char U+016A (decimal 362)
   defining Unicode char U+016B (decimal 363)
   defining Unicode char U+016C (decimal 364)
   defining Unicode char U+016D (decimal 365)
   defining Unicode char U+016E (decimal 366)
   defining Unicode char U+016F (decimal 367)
   defining Unicode char U+0170 (decimal 368)
   defining Unicode char U+0171 (decimal 369)
   defining Unicode char U+0172 (decimal 370)
   defining Unicode char U+0173 (decimal 371)
   defining Unicode char U+0174 (decimal 372)
   defining Unicode char U+0175 (decimal 373)
   defining Unicode char U+0176 (decimal 374)
   defining Unicode char U+0177 (decimal 375)
   defining Unicode char U+0178 (decimal 376)
   defining Unicode char U+0179 (decimal 377)
   defining Unicode char U+017A (decimal 378)
   defining Unicode char U+017B (decimal 379)
   defining Unicode char U+017C (decimal 380)
   defining Unicode char U+017D (decimal 381)
   defining Unicode char U+017E (decimal 382)
   defining Unicode char U+01CD (decimal 461)
   defining Unicode char U+01CE (decimal 462)
   defining Unicode char U+01CF (decimal 463)
   defining Unicode char U+01D0 (decimal 464)
   defining Unicode char U+01D1 (decimal 465)
   defining Unicode char U+01D2 (decimal 466)
   defining Unicode char U+01D3 (decimal 467)
   defining Unicode char U+01D4 (decimal 468)
   defining Unicode char U+01E2 (decimal 482)
   defining Unicode char U+01E3 (decimal 483)
   defining Unicode char U+01E6 (decimal 486)
   defining Unicode char U+01E7 (decimal 487)
   defining Unicode char U+01E8 (decimal 488)
   defining Unicode char U+01E9 (decimal 489)
   defining Unicode char U+01EA (decimal 490)
   defining Unicode char U+01EB (decimal 491)
   defining Unicode char U+01F0 (decimal 496)
   defining Unicode char U+01F4 (decimal 500)
   defining Unicode char U+01F5 (decimal 501)
   defining Unicode char U+0218 (decimal 536)
   defining Unicode char U+0219 (decimal 537)
   defining Unicode char U+021A (decimal 538)
   defining Unicode char U+021B (decimal 539)
   defining Unicode char U+0232 (decimal 562)
   defining Unicode char U+0233 (decimal 563)
   defining Unicode char U+1E02 (decimal 7682)
   defining Unicode char U+1E03 (decimal 7683)
   defining Unicode char U+200C (decimal 8204)
   defining Unicode char U+2010 (decimal 8208)
   defining Unicode char U+2011 (decimal 8209)
   defining Unicode char U+2012 (decimal 8210)
   defining Unicode char U+2013 (decimal 8211)
   defining Unicode char U+2014 (decimal 8212)
   defining Unicode char U+2015 (decimal 8213)
   defining Unicode char U+2018 (decimal 8216)
   defining Unicode char U+2019 (decimal 8217)
   defining Unicode char U+201A (decimal 8218)
   defining Unicode char U+201C (decimal 8220)
   defining Unicode char U+201D (decimal 8221)
   defining Unicode char U+201E (decimal 8222)
   defining Unicode char U+2030 (decimal 8240)
   defining Unicode char U+2031 (decimal 8241)
   defining Unicode char U+2039 (decimal 8249)
   defining Unicode char U+203A (decimal 8250)
   defining Unicode char U+2423 (decimal 9251)
   defining Unicode char U+1E20 (decimal 7712)
   defining Unicode char U+1E21 (decimal 7713)
)
Now handling font encoding OT1 ...
... processing UTF-8 mapping file for font encoding OT1

("C:\Program Files\MiKTeX 2.9\tex\latex\base\ot1enc.dfu"
File: ot1enc.dfu 2017/01/28 v1.1t UTF-8 support for inputenc
   defining Unicode char U+00A0 (decimal 160)
   defining Unicode char U+00A1 (decimal 161)
   defining Unicode char U+00A3 (decimal 163)
   defining Unicode char U+00AD (decimal 173)
   defining Unicode char U+00B8 (decimal 184)
   defining Unicode char U+00BF (decimal 191)
   defining Unicode char U+00C5 (decimal 197)
   defining Unicode char U+00C6 (decimal 198)
   defining Unicode char U+00D8 (decimal 216)
   defining Unicode char U+00DF (decimal 223)
   defining Unicode char U+00E6 (decimal 230)
   defining Unicode char U+00EC (decimal 236)
   defining Unicode char U+00ED (decimal 237)
   defining Unicode char U+00EE (decimal 238)
   defining Unicode char U+00EF (decimal 239)
   defining Unicode char U+00F8 (decimal 248)
   defining Unicode char U+0131 (decimal 305)
   defining Unicode char U+0141 (decimal 321)
   defining Unicode char U+0142 (decimal 322)
   defining Unicode char U+0152 (decimal 338)
   defining Unicode char U+0153 (decimal 339)
   defining Unicode char U+0174 (decimal 372)
   defining Unicode char U+0175 (decimal 373)
   defining Unicode char U+0176 (decimal 374)
   defining Unicode char U+0177 (decimal 375)
   defining Unicode char U+0218 (decimal 536)
   defining Unicode char U+0219 (decimal 537)
   defining Unicode char U+021A (decimal 538)
   defining Unicode char U+021B (decimal 539)
   defining Unicode char U+2013 (decimal 8211)
   defining Unicode char U+2014 (decimal 8212)
   defining Unicode char U+2018 (decimal 8216)
   defining Unicode char U+2019 (decimal 8217)
   defining Unicode char U+201C (decimal 8220)
   defining Unicode char U+201D (decimal 8221)
)
Now handling font encoding OMS ...
... processing UTF-8 mapping file for font encoding OMS

("C:\Program Files\MiKTeX 2.9\tex\latex\base\omsenc.dfu"
File: omsenc.dfu 2017/01/28 v1.1t UTF-8 support for inputenc
   defining Unicode char U+00A7 (decimal 167)
   defining Unicode char U+00B6 (decimal 182)
   defining Unicode char U+00B7 (decimal 183)
   defining Unicode char U+2020 (decimal 8224)
   defining Unicode char U+2021 (decimal 8225)
   defining Unicode char U+2022 (decimal 8226)
)
Now handling font encoding OMX ...
... no UTF-8 mapping file for font encoding OMX
Now handling font encoding U ...
... no UTF-8 mapping file for font encoding U
   defining Unicode char U+00A9 (decimal 169)
   defining Unicode char U+00AA (decimal 170)
   defining Unicode char U+00AE (decimal 174)
   defining Unicode char U+00BA (decimal 186)
   defining Unicode char U+02C6 (decimal 710)
   defining Unicode char U+02DC (decimal 732)
   defining Unicode char U+200C (decimal 8204)
   defining Unicode char U+2026 (decimal 8230)
   defining Unicode char U+2122 (decimal 8482)
   defining Unicode char U+2423 (decimal 9251)
))
("C:\Program Files\MiKTeX 2.9\tex\latex\microtype\microtype.sty"
Package: microtype 2017/07/07 v2.7 Micro-typographical refinements (RS)
\MT@toks=\toks17
\MT@count=\count89
LaTeX Info: Redefining \textls on input line 789.
\MT@outer@kern=\dimen104
LaTeX Info: Redefining \textmicrotypecontext on input line 1334.
\MT@listname@count=\count90

("C:\Program Files\MiKTeX 2.9\tex\latex\microtype\microtype-pdftex.def"
File: microtype-pdftex.def 2017/07/07 v2.7 Definitions specific to pdftex (RS)
LaTeX Info: Redefining \lsstyle on input line 912.
LaTeX Info: Redefining \lslig on input line 912.
\MT@outer@space=\skip55
)
Package microtype Info: Loading configuration file microtype.cfg.

("C:\Program Files\MiKTeX 2.9\tex\latex\microtype\microtype.cfg"
File: microtype.cfg 2017/07/07 v2.7 microtype main configuration file (RS)
))
("C:\Program Files\MiKTeX 2.9\tex\latex\tabu\tabu.sty"
Package: tabu 2011/02/26 v2.8 - flexible LaTeX tabulars (FC)

("C:\Program Files\MiKTeX 2.9\tex\latex\tools\array.sty"
Package: array 2016/10/06 v2.4d Tabular extension package (FMi)
\col@sep=\dimen105
\extrarowheight=\dimen106
\NC@list=\toks18
\extratabsurround=\skip56
\backup@length=\skip57
)
("C:\Program Files\MiKTeX 2.9\tex\latex\ltxmisc\varwidth.sty"
Package: varwidth 2009/03/30 ver 0.92;  Variable-width minipages
\@vwid@box=\box28
\sift@deathcycles=\count91
\@vwid@loff=\dimen107
\@vwid@roff=\dimen108
)
\c@taburow=\count92
\tabu@nbcols=\count93
\tabu@cnt=\count94
\tabu@Xcol=\count95
\tabu@alloc=\count96
\tabu@nested=\count97
\tabu@target=\dimen109
\tabu@spreadtarget=\dimen110
\tabu@naturalX=\dimen111
\tabucolX=\dimen112
\tabu@Xsum=\dimen113
\extrarowdepth=\dimen114
\abovetabulinesep=\dimen115
\belowtabulinesep=\dimen116
\tabustrutrule=\dimen117
\tabu@thebody=\toks19
\tabu@footnotes=\toks20
\tabu@box=\box29
\tabu@arstrutbox=\box30
\tabu@hleads=\box31
\tabu@vleads=\box32
\tabu@cellskip=\skip58
)
("C:\Program Files\MiKTeX 2.9\tex\latex\xcolor\xcolor.sty"
Package: xcolor 2016/05/11 v2.12 LaTeX color extensions (UK)

("C:\Program Files\MiKTeX 2.9\tex\latex\graphics-cfg\color.cfg"
File: color.cfg 2016/01/02 v1.6 sample color configuration
)
Package xcolor Info: Driver file: pdftex.def on input line 225.

("C:\Program Files\MiKTeX 2.9\tex\latex\graphics-def\pdftex.def"
File: pdftex.def 2017/06/24 v1.0g Graphics/color driver for pdftex
)
("C:\Program Files\MiKTeX 2.9\tex\latex\colortbl\colortbl.sty"
Package: colortbl 2012/02/13 v1.0a Color table columns (DPC)
\everycr=\toks21
\minrowclearance=\skip59
)
\rownum=\count98
Package xcolor Info: Model `cmy' substituted by `cmy0' on input line 1348.
Package xcolor Info: Model `hsb' substituted by `rgb' on input line 1352.
Package xcolor Info: Model `RGB' extended on input line 1364.
Package xcolor Info: Model `HTML' substituted by `rgb' on input line 1366.
Package xcolor Info: Model `Hsb' substituted by `hsb' on input line 1367.
Package xcolor Info: Model `tHsb' substituted by `hsb' on input line 1368.
Package xcolor Info: Model `HSB' substituted by `hsb' on input line 1369.
Package xcolor Info: Model `Gray' substituted by `gray' on input line 1370.
Package xcolor Info: Model `wave' substituted by `hsb' on input line 1371.

("C:\Program Files\MiKTeX 2.9\tex\latex\graphics\dvipsnam.def"
File: dvipsnam.def 2016/06/17 v3.0m Driver-dependent file (DPC,SPQR)
)
("C:\Program Files\MiKTeX 2.9\tex\latex\xcolor\x11nam.def"
File: x11nam.def 2016/05/11 v2.12 Predefined colors according to Unix/X11 (UK)
))
("C:\Program Files\MiKTeX 2.9\tex\latex\amsmath\amsmath.sty"
Package: amsmath 2016/11/05 v2.16a AMS math features
\@mathmargin=\skip60

For additional information on amsmath, use the `?' option.
("C:\Program Files\MiKTeX 2.9\tex\latex\amsmath\amstext.sty"
Package: amstext 2000/06/29 v2.01 AMS text

("C:\Program Files\MiKTeX 2.9\tex\latex\amsmath\amsgen.sty"
File: amsgen.sty 1999/11/30 v2.0 generic functions
\@emptytoks=\toks22
\ex@=\dimen118
))
("C:\Program Files\MiKTeX 2.9\tex\latex\amsmath\amsbsy.sty"
Package: amsbsy 1999/11/29 v1.2d Bold Symbols
\pmbraise@=\dimen119
)
("C:\Program Files\MiKTeX 2.9\tex\latex\amsmath\amsopn.sty"
Package: amsopn 2016/03/08 v2.02 operator names
)
\inf@bad=\count99
LaTeX Info: Redefining \frac on input line 213.
\uproot@=\count100
\leftroot@=\count101
LaTeX Info: Redefining \overline on input line 375.
\classnum@=\count102
\DOTSCASE@=\count103
LaTeX Info: Redefining \ldots on input line 472.
LaTeX Info: Redefining \dots on input line 475.
LaTeX Info: Redefining \cdots on input line 596.
\Mathstrutbox@=\box33
\strutbox@=\box34
\big@size=\dimen120
LaTeX Font Info:    Redeclaring font encoding OML on input line 712.
LaTeX Font Info:    Redeclaring font encoding OMS on input line 713.
\macc@depth=\count104
\c@MaxMatrixCols=\count105
\dotsspace@=\muskip10
\c@parentequation=\count106
\dspbrk@lvl=\count107
\tag@help=\toks23
\row@=\count108
\column@=\count109
\maxfields@=\count110
\andhelp@=\toks24
\eqnshift@=\dimen121
\alignsep@=\dimen122
\tagshift@=\dimen123
\tagwidth@=\dimen124
\totwidth@=\dimen125
\lineht@=\dimen126
\@envbody=\toks25
\multlinegap=\skip61
\multlinetaggap=\skip62
\mathdisplay@stack=\toks26
LaTeX Info: Redefining \[ on input line 2817.
LaTeX Info: Redefining \] on input line 2818.
)
("C:\Program Files\MiKTeX 2.9\tex\latex\caption\caption.sty"
Package: caption 2016/02/21 v3.3-144 Customizing captions (AR)

("C:\Program Files\MiKTeX 2.9\tex\latex\caption\caption3.sty"
Package: caption3 2016/05/22 v1.7-166 caption3 kernel (AR)
Package caption3 Info: TeX engine: e-TeX on input line 67.
\captionmargin=\dimen127
\captionmargin@=\dimen128
\captionwidth=\dimen129
\caption@tempdima=\dimen130
\caption@indent=\dimen131
\caption@parindent=\dimen132
\caption@hangindent=\dimen133
)
Package caption Info: KOMA-Script document class.
\c@ContinuedFloat=\count111
)
("C:\Program Files\MiKTeX 2.9\tex\latex\graphics\graphicx.sty"
Package: graphicx 2017/06/01 v1.1a Enhanced LaTeX Graphics (DPC,SPQR)

("C:\Program Files\MiKTeX 2.9\tex\latex\graphics\graphics.sty"
Package: graphics 2017/06/25 v1.2c Standard LaTeX Graphics (DPC,SPQR)

("C:\Program Files\MiKTeX 2.9\tex\latex\graphics\trig.sty"
Package: trig 2016/01/03 v1.10 sin cos tan (DPC)
)
("C:\Program Files\MiKTeX 2.9\tex\latex\graphics-cfg\graphics.cfg"
File: graphics.cfg 2016/06/04 v1.11 sample graphics configuration
)
Package graphics Info: Driver file: pdftex.def on input line 99.
)
\Gin@req@height=\dimen134
\Gin@req@width=\dimen135
)
("C:\Program Files\MiKTeX 2.9\tex\latex\hyperref\hyperref.sty"
Package: hyperref 2017/03/14 v6.85a Hypertext links for LaTeX

("C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\hobsub-hyperref.sty"
Package: hobsub-hyperref 2016/05/16 v1.14 Bundle oberdiek, subset hyperref (HO)


("C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\hobsub-generic.sty"
Package: hobsub-generic 2016/05/16 v1.14 Bundle oberdiek, subset generic (HO)
Package: hobsub 2016/05/16 v1.14 Construct package bundles (HO)
Package: infwarerr 2016/05/16 v1.4 Providing info/warning/error messages (HO)
Package: ltxcmds 2016/05/16 v1.23 LaTeX kernel commands for general use (HO)
Package: ifluatex 2016/05/16 v1.4 Provides the ifluatex switch (HO)
Package ifluatex Info: LuaTeX not detected.
Package: ifvtex 2016/05/16 v1.6 Detect VTeX and its facilities (HO)
Package ifvtex Info: VTeX not detected.
Package: intcalc 2016/05/16 v1.2 Expandable calculations with integers (HO)
Package: ifpdf 2017/03/15 v3.2 Provides the ifpdf switch
Package: etexcmds 2016/05/16 v1.6 Avoid name clashes with e-TeX commands (HO)
Package etexcmds Info: Could not find \expanded.
(etexcmds)             That can mean that you are not using pdfTeX 1.50 or
(etexcmds)             that some package has redefined \expanded.
(etexcmds)             In the latter case, load this package earlier.
Package: kvsetkeys 2016/05/16 v1.17 Key value parser (HO)
Package: kvdefinekeys 2016/05/16 v1.4 Define keys (HO)
Package: pdftexcmds 2017/03/19 v0.25 Utility functions of pdfTeX for LuaTeX (HO
)
Package pdftexcmds Info: LuaTeX not detected.
Package pdftexcmds Info: \pdf@primitive is available.
Package pdftexcmds Info: \pdf@ifprimitive is available.
Package pdftexcmds Info: \pdfdraftmode found.
Package: pdfescape 2016/05/16 v1.14 Implements pdfTeX's escape features (HO)
Package: bigintcalc 2016/05/16 v1.4 Expandable calculations on big integers (HO
)
Package: bitset 2016/05/16 v1.2 Handle bit-vector datatype (HO)
Package: uniquecounter 2016/05/16 v1.3 Provide unlimited unique counter (HO)
)
Package hobsub Info: Skipping package `hobsub' (already loaded).
Package: letltxmacro 2016/05/16 v1.5 Let assignment for LaTeX macros (HO)
Package: hopatch 2016/05/16 v1.3 Wrapper for package hooks (HO)
Package: xcolor-patch 2016/05/16 xcolor patch
Package: atveryend 2016/05/16 v1.9 Hooks at the very end of document (HO)
Package atveryend Info: \enddocument detected (standard20110627).
Package: atbegshi 2016/06/09 v1.18 At begin shipout hook (HO)
Package: refcount 2016/05/16 v3.5 Data extraction from label references (HO)
Package: hycolor 2016/05/16 v1.8 Color options for hyperref/bookmark (HO)
)
("C:\Program Files\MiKTeX 2.9\tex\generic\ifxetex\ifxetex.sty"
Package: ifxetex 2010/09/12 v0.6 Provides ifxetex conditional
)
("C:\Program Files\MiKTeX 2.9\tex\latex\oberdiek\auxhook.sty"
Package: auxhook 2016/05/16 v1.4 Hooks for auxiliary files (HO)
)
("C:\Program Files\MiKTeX 2.9\tex\latex\oberdiek\kvoptions.sty"
Package: kvoptions 2016/05/16 v3.12 Key value format for package options (HO)
)
\@linkdim=\dimen136
\Hy@linkcounter=\count112
\Hy@pagecounter=\count113

("C:\Program Files\MiKTeX 2.9\tex\latex\hyperref\pd1enc.def"
File: pd1enc.def 2017/03/14 v6.85a Hyperref: PDFDocEncoding definition (HO)
Now handling font encoding PD1 ...
... no UTF-8 mapping file for font encoding PD1
)
\Hy@SavedSpaceFactor=\count114

("C:\Program Files\MiKTeX 2.9\tex\latex\00miktex\hyperref.cfg"
File: hyperref.cfg 2002/06/06 v1.2 hyperref configuration of TeXLive
)
Package hyperref Info: Hyper figures OFF on input line 4498.
Package hyperref Info: Link nesting OFF on input line 4503.
Package hyperref Info: Hyper index ON on input line 4506.
Package hyperref Info: Plain pages OFF on input line 4513.
Package hyperref Info: Backreferencing OFF on input line 4518.
Package hyperref Info: Implicit mode ON; LaTeX internals redefined.
Package hyperref Info: Bookmarks ON on input line 4751.
\c@Hy@tempcnt=\count115

("C:\Program Files\MiKTeX 2.9\tex\latex\url\url.sty"
\Urlmuskip=\muskip11
Package: url 2013/09/16  ver 3.4  Verb mode for urls, etc.
)
LaTeX Info: Redefining \url on input line 5104.
\XeTeXLinkMargin=\dimen137
\Fld@menulength=\count116
\Field@Width=\dimen138
\Fld@charsize=\dimen139
Package hyperref Info: Hyper figures OFF on input line 6358.
Package hyperref Info: Link nesting OFF on input line 6363.
Package hyperref Info: Hyper index ON on input line 6366.
Package hyperref Info: backreferencing OFF on input line 6373.
Package hyperref Info: Link coloring OFF on input line 6378.
Package hyperref Info: Link coloring with OCG OFF on input line 6383.
Package hyperref Info: PDF/A mode OFF on input line 6388.
LaTeX Info: Redefining \ref on input line 6428.
LaTeX Info: Redefining \pageref on input line 6432.
\Hy@abspage=\count117
\c@Item=\count118
\c@Hfootnote=\count119
)

Package hyperref Message: Driver (autodetected): hpdftex.

("C:\Program Files\MiKTeX 2.9\tex\latex\hyperref\hpdftex.def"
File: hpdftex.def 2017/03/14 v6.85a Hyperref driver for pdfTeX
\Fld@listcount=\count120
\c@bookmark@seq@number=\count121

("C:\Program Files\MiKTeX 2.9\tex\latex\oberdiek\rerunfilecheck.sty"
Package: rerunfilecheck 2016/05/16 v1.8 Rerun checks for auxiliary files (HO)
Package uniquecounter Info: New unique counter `rerunfilecheck' on input line 2
82.
)
\Hy@SectionHShift=\skip63
)
("C:\Program Files\MiKTeX 2.9\tex\latex\cleveref\cleveref.sty"
Package: cleveref 2013/12/28 v0.19 Intelligent cross-referencing
Package cleveref Info: `hyperref' support loaded on input line 2230.
LaTeX Info: Redefining \cref on input line 2230.
LaTeX Info: Redefining \Cref on input line 2230.
LaTeX Info: Redefining \crefrange on input line 2230.
LaTeX Info: Redefining \Crefrange on input line 2230.
LaTeX Info: Redefining \cpageref on input line 2230.
LaTeX Info: Redefining \Cpageref on input line 2230.
LaTeX Info: Redefining \cpagerefrange on input line 2230.
LaTeX Info: Redefining \Cpagerefrange on input line 2230.
LaTeX Info: Redefining \labelcref on input line 2230.
LaTeX Info: Redefining \labelcpageref on input line 2230.
)
("C:\Program Files\MiKTeX 2.9\tex\latex\tools\bm.sty"
Package: bm 2017/01/16 v1.2c Bold Symbol Support (DPC/FMi)
\symboldoperators=\mathgroup4
\symboldletters=\mathgroup5
\symboldsymbols=\mathgroup6
LaTeX Font Info:    Redeclaring math alphabet \mathbf on input line 141.
LaTeX Info: Redefining \bm on input line 207.
)
("C:\Program Files\MiKTeX 2.9\tex\latex\amsfonts\amsfonts.sty"
Package: amsfonts 2013/01/14 v3.01 Basic AMSFonts support
\symAMSa=\mathgroup7
\symAMSb=\mathgroup8
LaTeX Font Info:    Overwriting math alphabet `\mathfrak' in version `bold'
(Font)                  U/euf/m/n --> U/euf/b/n on input line 106.
)
("C:\Program Files\MiKTeX 2.9\tex\latex\pgf\frontendlayer\tikz.sty"
("C:\Program Files\MiKTeX 2.9\tex\latex\pgf\basiclayer\pgf.sty"
("C:\Program Files\MiKTeX 2.9\tex\latex\pgf\utilities\pgfrcs.sty"
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\utilities\pgfutil-common.tex"
\pgfutil@everybye=\toks27
\pgfutil@tempdima=\dimen140
\pgfutil@tempdimb=\dimen141

("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\utilities\pgfutil-common-lists.te
x")) ("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\utilities\pgfutil-latex.def"
\pgfutil@abb=\box35
("C:\Program Files\MiKTeX 2.9\tex\latex\ms\everyshi.sty"
Package: everyshi 2001/05/15 v3.00 EveryShipout Package (MS)
))
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\utilities\pgfrcs.code.tex"
Package: pgfrcs 2015/08/07 v3.0.1a (rcs-revision 1.31)
))
Package: pgf 2015/08/07 v3.0.1a (rcs-revision 1.15)

("C:\Program Files\MiKTeX 2.9\tex\latex\pgf\basiclayer\pgfcore.sty"
("C:\Program Files\MiKTeX 2.9\tex\latex\pgf\systemlayer\pgfsys.sty"
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\systemlayer\pgfsys.code.tex"
Package: pgfsys 2014/07/09 v3.0.1a (rcs-revision 1.48)

("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\utilities\pgfkeys.code.tex"
\pgfkeys@pathtoks=\toks28
\pgfkeys@temptoks=\toks29

("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\utilities\pgfkeysfiltered.code.te
x"
\pgfkeys@tmptoks=\toks30
))
\pgf@x=\dimen142
\pgf@y=\dimen143
\pgf@xa=\dimen144
\pgf@ya=\dimen145
\pgf@xb=\dimen146
\pgf@yb=\dimen147
\pgf@xc=\dimen148
\pgf@yc=\dimen149
\w@pgf@writea=\write3
\r@pgf@reada=\read1
\c@pgf@counta=\count122
\c@pgf@countb=\count123
\c@pgf@countc=\count124
\c@pgf@countd=\count125
\t@pgf@toka=\toks31
\t@pgf@tokb=\toks32
\t@pgf@tokc=\toks33
 ("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\systemlayer\pgf.cfg"
File: pgf.cfg 2008/05/14  (rcs-revision 1.7)
)
Driver file for pgf: pgfsys-pdftex.def

("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\systemlayer\pgfsys-pdftex.def"
File: pgfsys-pdftex.def 2014/10/11  (rcs-revision 1.35)

("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\systemlayer\pgfsys-common-pdf.def
"
File: pgfsys-common-pdf.def 2013/10/10  (rcs-revision 1.13)
)))
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\systemlayer\pgfsyssoftpath.code.t
ex"
File: pgfsyssoftpath.code.tex 2013/09/09  (rcs-revision 1.9)
\pgfsyssoftpath@smallbuffer@items=\count126
\pgfsyssoftpath@bigbuffer@items=\count127
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\systemlayer\pgfsysprotocol.code.t
ex"
File: pgfsysprotocol.code.tex 2006/10/16  (rcs-revision 1.4)
)) ("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcore.code.tex"
Package: pgfcore 2010/04/11 v3.0.1a (rcs-revision 1.7)
 ("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmath.code.tex"
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathcalc.code.tex"
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathutil.code.tex")
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathparser.code.tex"
\pgfmath@dimen=\dimen150
\pgfmath@count=\count128
\pgfmath@box=\box36
\pgfmath@toks=\toks34
\pgfmath@stack@operand=\toks35
\pgfmath@stack@operation=\toks36
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.code.tex"
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.basic.code.
tex")
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.trigonometr
ic.code.tex")
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.random.code
.tex")
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.comparison.
code.tex")
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.base.code.t
ex")
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.round.code.
tex")
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.misc.code.t
ex")
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.integerarit
hmetics.code.tex")))
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfloat.code.tex"
\c@pgfmathroundto@lastzeros=\count129
))
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorepoints.code.tex
"
File: pgfcorepoints.code.tex 2013/10/07  (rcs-revision 1.27)
\pgf@picminx=\dimen151
\pgf@picmaxx=\dimen152
\pgf@picminy=\dimen153
\pgf@picmaxy=\dimen154
\pgf@pathminx=\dimen155
\pgf@pathmaxx=\dimen156
\pgf@pathminy=\dimen157
\pgf@pathmaxy=\dimen158
\pgf@xx=\dimen159
\pgf@xy=\dimen160
\pgf@yx=\dimen161
\pgf@yy=\dimen162
\pgf@zx=\dimen163
\pgf@zy=\dimen164
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorepathconstruct.c
ode.tex"
File: pgfcorepathconstruct.code.tex 2013/10/07  (rcs-revision 1.29)
\pgf@path@lastx=\dimen165
\pgf@path@lasty=\dimen166
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorepathusage.code.
tex"
File: pgfcorepathusage.code.tex 2014/11/02  (rcs-revision 1.24)
\pgf@shorten@end@additional=\dimen167
\pgf@shorten@start@additional=\dimen168
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorescopes.code.tex
"
File: pgfcorescopes.code.tex 2015/05/08  (rcs-revision 1.46)
\pgfpic=\box37
\pgf@hbox=\box38
\pgf@layerbox@main=\box39
\pgf@picture@serial@count=\count130
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcoregraphicstate.co
de.tex"
File: pgfcoregraphicstate.code.tex 2014/11/02  (rcs-revision 1.12)
\pgflinewidth=\dimen169
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcoretransformations
.code.tex"
File: pgfcoretransformations.code.tex 2015/08/07  (rcs-revision 1.20)
\pgf@pt@x=\dimen170
\pgf@pt@y=\dimen171
\pgf@pt@temp=\dimen172
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorequick.code.tex"
File: pgfcorequick.code.tex 2008/10/09  (rcs-revision 1.3)
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcoreobjects.code.te
x"
File: pgfcoreobjects.code.tex 2006/10/11  (rcs-revision 1.2)
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorepathprocessing.
code.tex"
File: pgfcorepathprocessing.code.tex 2013/09/09  (rcs-revision 1.9)
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorearrows.code.tex
"
File: pgfcorearrows.code.tex 2015/05/14  (rcs-revision 1.43)
\pgfarrowsep=\dimen173
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcoreshade.code.tex"
File: pgfcoreshade.code.tex 2013/07/15  (rcs-revision 1.15)
\pgf@max=\dimen174
\pgf@sys@shading@range@num=\count131
) ("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcoreimage.code.te
x"
File: pgfcoreimage.code.tex 2013/07/15  (rcs-revision 1.18)

("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcoreexternal.code.t
ex"
File: pgfcoreexternal.code.tex 2014/07/09  (rcs-revision 1.21)
\pgfexternal@startupbox=\box40
))
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorelayers.code.tex
"
File: pgfcorelayers.code.tex 2013/07/18  (rcs-revision 1.7)
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcoretransparency.co
de.tex"
File: pgfcoretransparency.code.tex 2013/09/30  (rcs-revision 1.5)
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorepatterns.code.t
ex"
File: pgfcorepatterns.code.tex 2013/11/07  (rcs-revision 1.5)
)))
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\modules\pgfmoduleshapes.code.tex"
File: pgfmoduleshapes.code.tex 2014/03/21  (rcs-revision 1.35)
\pgfnodeparttextbox=\box41
) ("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\modules\pgfmoduleplot.code.tex"
File: pgfmoduleplot.code.tex 2015/08/03  (rcs-revision 1.13)
)
("C:\Program Files\MiKTeX 2.9\tex\latex\pgf\compatibility\pgfcomp-version-0-65.
sty"
Package: pgfcomp-version-0-65 2007/07/03 v3.0.1a (rcs-revision 1.7)
\pgf@nodesepstart=\dimen175
\pgf@nodesepend=\dimen176
)
("C:\Program Files\MiKTeX 2.9\tex\latex\pgf\compatibility\pgfcomp-version-1-18.
sty"
Package: pgfcomp-version-1-18 2007/07/23 v3.0.1a (rcs-revision 1.1)
)) ("C:\Program Files\MiKTeX 2.9\tex\latex\pgf\utilities\pgffor.sty"
("C:\Program Files\MiKTeX 2.9\tex\latex\pgf\utilities\pgfkeys.sty"
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\utilities\pgfkeys.code.tex"))
("C:\Program Files\MiKTeX 2.9\tex\latex\pgf\math\pgfmath.sty"
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmath.code.tex"))
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\utilities\pgffor.code.tex"
Package: pgffor 2013/12/13 v3.0.1a (rcs-revision 1.25)

("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmath.code.tex")
\pgffor@iter=\dimen177
\pgffor@skip=\dimen178
\pgffor@stack=\toks37
\pgffor@toks=\toks38
))
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\frontendlayer\tikz\tikz.code.tex"
Package: tikz 2015/08/07 v3.0.1a (rcs-revision 1.151)

("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\libraries\pgflibraryplothandlers.
code.tex"
File: pgflibraryplothandlers.code.tex 2013/08/31 v3.0.1a (rcs-revision 1.20)
\pgf@plot@mark@count=\count132
\pgfplotmarksize=\dimen179
)
\tikz@lastx=\dimen180
\tikz@lasty=\dimen181
\tikz@lastxsaved=\dimen182
\tikz@lastysaved=\dimen183
\tikzleveldistance=\dimen184
\tikzsiblingdistance=\dimen185
\tikz@figbox=\box42
\tikz@figbox@bg=\box43
\tikz@tempbox=\box44
\tikz@tempbox@bg=\box45
\tikztreelevel=\count133
\tikznumberofchildren=\count134
\tikznumberofcurrentchild=\count135
\tikz@fig@count=\count136

("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\modules\pgfmodulematrix.code.tex"
File: pgfmodulematrix.code.tex 2013/09/17  (rcs-revision 1.8)
\pgfmatrixcurrentrow=\count137
\pgfmatrixcurrentcolumn=\count138
\pgf@matrix@numberofcolumns=\count139
)
\tikz@expandcount=\count140

("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\frontendlayer\tikz\libraries\tikz
librarytopaths.code.tex"
File: tikzlibrarytopaths.code.tex 2008/06/17 v3.0.1a (rcs-revision 1.2)
)))
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\frontendlayer\tikz\libraries\tikz
libraryshapes.geometric.code.tex"
File: tikzlibraryshapes.geometric.code.tex 2008/01/09 v3.0.1a (rcs-revision 1.1
)

("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\libraries\shapes\pgflibraryshapes
.geometric.code.tex"
File: pgflibraryshapes.geometric.code.tex 2008/06/26 v3.0.1a (rcs-revision 1.1)

))
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\frontendlayer\tikz\libraries\tikz
libraryarrows.code.tex"
File: tikzlibraryarrows.code.tex 2008/01/09 v3.0.1a (rcs-revision 1.1)

("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\libraries\pgflibraryarrows.code.t
ex"
File: pgflibraryarrows.code.tex 2013/09/23 v3.0.1a (rcs-revision 1.16)
\arrowsize=\dimen186
))
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\frontendlayer\tikz\libraries\tikz
librarycalc.code.tex"
File: tikzlibrarycalc.code.tex 2013/07/15 v3.0.1a (rcs-revision 1.9)
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\frontendlayer\tikz\libraries\tikz
librarypositioning.code.tex"
File: tikzlibrarypositioning.code.tex 2008/10/06 v3.0.1a (rcs-revision 1.7)
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\libraries\pgflibraryarrows.meta.c
ode.tex"
File: pgflibraryarrows.meta.code.tex 2015/05/13 v3.0.1a (rcs-revision 1.13)
\pgfarrowinset=\dimen187
\pgfarrowlength=\dimen188
\pgfarrowwidth=\dimen189
\pgfarrowlinewidth=\dimen190
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\frontendlayer\tikz\libraries\tikz
librarydecorations.code.tex"
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\modules\pgfmoduledecorations.code
.tex"
\pgfdecoratedcompleteddistance=\dimen191
\pgfdecoratedremainingdistance=\dimen192
\pgfdecoratedinputsegmentcompleteddistance=\dimen193
\pgfdecoratedinputsegmentremainingdistance=\dimen194
\pgf@decorate@distancetomove=\dimen195
\pgf@decorate@repeatstate=\count141
\pgfdecorationsegmentamplitude=\dimen196
\pgfdecorationsegmentlength=\dimen197
)
\tikz@lib@dec@box=\box46
)
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\frontendlayer\tikz\libraries\tikz
librarydecorations.pathmorphing.code.tex"
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\libraries\decorations\pgflibraryd
ecorations.pathmorphing.code.tex"))
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\frontendlayer\tikz\libraries\tikz
librarydecorations.pathreplacing.code.tex"
("C:\Program Files\MiKTeX 2.9\tex\generic\pgf\libraries\decorations\pgflibraryd
ecorations.pathreplacing.code.tex"))
("C:\Program Files\MiKTeX 2.9\tex\latex\algorithms\algorithm.sty"
Package: algorithm 2009/08/24 v0.1 Document Style `algorithm' - floating enviro
nment

("C:\Program Files\MiKTeX 2.9\tex\latex\float\float.sty"
Package: float 2001/11/08 v1.3d Float enhancements (AL)
\c@float@type=\count142
\float@exts=\toks39
\float@box=\box47
\@float@everytoks=\toks40
\@floatcapt=\box48
)
("C:\Program Files\MiKTeX 2.9\tex\latex\base\ifthen.sty"
Package: ifthen 2014/09/29 v1.1c Standard LaTeX ifthen package (DPC)
)
\@float@every@algorithm=\toks41
\c@algorithm=\count143
)
("C:\Program Files\MiKTeX 2.9\tex\latex\algorithmicx\algpseudocode.sty"
Package: algpseudocode 

("C:\Program Files\MiKTeX 2.9\tex\latex\algorithmicx\algorithmicx.sty"
Package: algorithmicx 2005/04/27 v1.2 Algorithmicx

Document Style algorithmicx 1.2 - a greatly improved `algorithmic' style
\c@ALG@line=\count144
\c@ALG@rem=\count145
\c@ALG@nested=\count146
\ALG@tlm=\skip64
\ALG@thistlm=\skip65
\c@ALG@Lnr=\count147
\c@ALG@blocknr=\count148
\c@ALG@storecount=\count149
\c@ALG@tmpcounter=\count150
\ALG@tmplength=\skip66
)
Document Style - pseudocode environments for use with the `algorithmicx' style
) (C:\ProgramData\texmfbosch\tex\latex\bosch\bosch.sty
Package: bosch 2018/02/13 v4.0.0 Bosch Corporate Design


Package: bosch, S. Simon, 2001-2018, 2018/02/13 v4.0.0 
Author:
 Stephan Simon (2001-2018)
with contributions from:
 Tobias Rad (2017-2018: SCCM package, TeX logo implementation)
 Christian Hoeppler (2016: Bosch Office Sans font)
 Florian Brucker (2013: Feber template)

(C:\ProgramData\texmfbosch\tex\latex\bosch\boschformat.sty
Package: boschformat 2018/02/13 v4.0.0 Bosch page formats

Package: boschformat, Stephan Simon, 2001-2018, 2018/02/13 v4.0.0 

("C:\Program Files\MiKTeX 2.9\tex\latex\etoolbox\etoolbox.sty"
Package: etoolbox 2017/01/02 v2.4 e-TeX tools for LaTeX (JAW)
\etb@tempcnta=\count151
)
("C:\Program Files\MiKTeX 2.9\tex\latex\tools\calc.sty"
Package: calc 2014/10/28 v4.3 Infix arithmetic (KKT,FJ)
\calc@Acount=\count152
\calc@Bcount=\count153
\calc@Adimen=\dimen198
\calc@Bdimen=\dimen199
\calc@Askip=\skip67
\calc@Bskip=\skip68
LaTeX Info: Redefining \setlength on input line 80.
LaTeX Info: Redefining \addtolength on input line 81.
\calc@Ccount=\count154
\calc@Cskip=\skip69
)
\dx=\skip70
\dy=\skip71
\dxymin=\skip72
\dxymax=\skip73
\dxyz=\skip74
\paperLongSide=\skip75
\paperShortSide=\skip76
\bordTop=\skip77
\bordBottom=\skip78
\bordLeft=\skip79
\bordRight=\skip80
\@RBlowerEdgeYpos=\skip81
\@RBpageDiag=\skip82
\RBhHgt=\skip83
\@RBlogoWdt=\skip84
\@RBlogoHgt=\skip85
\@RBlogoXpos=\skip86
\@RBlogoYpos=\skip87
\@RBlifeClipWdt=\skip88
\@RBlifeClipHgt=\skip89
\@RBlifeClipXpos=\skip90
\@RBlifeClipYpos=\skip91
\@RBmyPicWdt=\skip92
\@RBmyPicHgt=\skip93
\@RBmyPicXpos=\skip94
\@RBmyPicYpos=\skip95
\@RBsgFullHgt=\skip96
\@RBsgWdt=\skip97
\@RBsgHgt=\skip98
\@RBsgXpos=\skip99
\@RBsgYpos=\skip100
\@RBbackWdt=\skip101
\@RBbackHgt=\skip102
\@RBbackXpos=\skip103
\@RBbackYpos=\skip104
\@RBtitleWdt=\skip105
\@RBtitleHgt=\skip106
\@RBtitleXpos=\skip107
\@RBtitleYpos=\skip108
\@RBtitleYmargin=\skip109
\@RBheadUsableHgt=\skip110
\@RBheadUsableYpos=\skip111
\@RBdataWdt=\skip112
\@RBdataHgt=\skip113
\@RBdataXpos=\skip114
\@RBdataYpos=\skip115
\@RBmyBackPicWdt=\skip116
\@RBmyBackPicHgt=\skip117
\@RBmyBackPicXpos=\skip118
\@RBmyBackPicYpos=\skip119
\@RBfootBoxXpos=\skip120
\@RBfootBoxYpos=\skip121
\@RBfootBoxWdt=\skip122
\@RBfootBoxHgt=\skip123
\TempRatioInPt=\skip124
)
boschformat: using A4 portrait paper format
Package typearea Info: These are the values describing the layout:
(typearea)             DIV  = 10
(typearea)             BCOR = 0.0pt
(typearea)             \paperwidth      = 598.14613pt
(typearea)              \textwidth      = 418.70232pt
(typearea)              DIV departure   = -7%
(typearea)              \evensidemargin = 17.45192pt
(typearea)              \oddsidemargin  = 17.45192pt
(typearea)             \paperheight     = 845.90547pt
(typearea)              \textheight     = 595.80026pt
(typearea)              \topmargin      = -25.07945pt
(typearea)              \headheight     = 17.0pt
(typearea)              \headsep        = 20.40001pt
(typearea)              \topskip        = 11.0pt
(typearea)              \footskip       = 47.6pt
(typearea)              \baselineskip   = 13.6pt
(typearea)              on input line 192.
("C:\Program Files\MiKTeX 2.9\tex\latex\oberdiek\transparent.sty"
Package: transparent 2016/05/16 v1.1 Transparency via pdfTeX's color stack (HO)

)
("C:\Program Files\MiKTeX 2.9\tex\latex\tools\xspace.sty"
Package: xspace 2014/10/28 v1.13 Space after command names (DPC,MH)
)
(C:\ProgramData\texmfbosch\tex\latex\bosch\boschlanguage.sty
Package: boschlanguage 2018/02/13 v4.0.0 Bosch elements

Package: boschlanguage, Stephan Simon, 2001-2017, 2018/02/13 v4.0.0 

) (C:\ProgramData\texmfbosch\tex\latex\bosch\boschcolors.sty
Package: boschcolors 2018/02/13 v4.0.0 Bosch corporate design colors

Package: boschcolors, Stephan Simon, 2001-2017, 2018/02/13 v4.0.0 

Provides recommended colors of Bosch Corporate Design 2016:
BoschFuchsia100, BoschFuchsia050, BoschViolet100, BoschViolet050, BoschDarkBlue
100, BoschDarkBlue050, BoschLightBlue100, BoschLightBlue050, BoschTurquoise100,
 BoschTurquoise050, BoschLightGreen100, BoschLightGreen050, BoschDarkGreen100, 
BoschDarkGreen050, BoschDarkGray, BoschLightGray, BoschRed, LinkColor

Old colors of Bosch Corporate Design 2006:
DO NOT USE! ONLY FOR BACKWARD COMPATIBILITY!
BoschBlue100, BoschBlue100CMYK, BoschBlue075, BoschBlue075CMYK, BoschBlue050, B
oschBlue050CMYK, BoschBlue025, BoschBlue025CMYK, BoschBlueNews, BoschRedOld, Bo
schRedOldCMYK, BoschGray, BoschGrayCMYK, BoschLightGrayOld, BoschLightGrayOldCM
YK, BoschBackgGrayCMYK, BoschLightBlue, BoschLightBlueCMYK, BoschRedBrown, Bosc
hRedBrownCMYK, BoschYellowGreen, BoschYellowGreenCMYK, BoschPTGreenCMYK

) (C:\ProgramData\texmfbosch\tex\latex\bosch\boschtools.sty
Package: boschtools 2018/02/13 v4.0.0 Bosch tools

Package: boschtools, Stephan Simon, 2001-2017, 2018/02/13 v4.0.0 

\@RBigDestWdt=\skip125
\@RBigDestHgt=\skip126
\@RBigTryWdtA=\skip127
\@RBigTryWdtB=\skip128
\@RBigCurrWdt=\skip129
\@RBigCurrHgt=\skip130
\@RBigCurrDpt=\skip131
\@RBigTrimL=\skip132
\@RBigTrimR=\skip133
\@RBigTrimLR=\skip134
\@RBigTrimB=\skip135
\@RBigTrimT=\skip136
\@RBigTrimBT=\skip137
\@RBigSaveBoxA=\box49
\@RBigSaveBoxB=\box50
) (C:\ProgramData\texmfbosch\tex\latex\bosch\boschelements.sty
Package: boschelements 2018/02/13 v4.0.0 Bosch elements

Package: boschelements, Stephan Simon, 2001-2018, 2018/02/13 v4.0.0 

("C:\Program Files\MiKTeX 2.9\tex\latex\adjustbox\adjustbox.sty"
Package: adjustbox 2012/05/21 v1.0 Adjusting TeX boxes (trim, clip, ...)

("C:\Program Files\MiKTeX 2.9\tex\latex\xkeyval\xkeyval.sty"
Package: xkeyval 2014/12/03 v2.7a package option processing (HA)

("C:\Program Files\MiKTeX 2.9\tex\generic\xkeyval\xkeyval.tex"
("C:\Program Files\MiKTeX 2.9\tex\generic\xkeyval\xkvutils.tex"
\XKV@toks=\toks42
\XKV@tempa@toks=\toks43
)
\XKV@depth=\count155
File: xkeyval.tex 2014/12/03 v2.7a key=value parser (HA)
))
("C:\Program Files\MiKTeX 2.9\tex\latex\adjustbox\adjcalc.sty"
Package: adjcalc 2012/05/16 v1.1 Provides advanced setlength with multiple back
-ends (calc, etex, pgfmath)
)
("C:\Program Files\MiKTeX 2.9\tex\latex\adjustbox\trimclip.sty"
Package: trimclip 2012/05/16 v1.0 Trim and clip general TeX material

("C:\Program Files\MiKTeX 2.9\tex\latex\collectbox\collectbox.sty"
Package: collectbox 2012/05/17 v0.4b Collect macro arguments as boxes
\collectedbox=\box51
)
\tc@llx=\dimen256
\tc@lly=\dimen257
\tc@urx=\dimen258
\tc@ury=\dimen259
Package trimclip Info: Using driver 'tc-pdftex.def'.

("C:\Program Files\MiKTeX 2.9\tex\latex\adjustbox\tc-pdftex.def"
File: tc-pdftex.def 2012/05/13 v1.0 Clipping driver for pdftex
))
\adjbox@Width=\dimen260
\adjbox@Height=\dimen261
\adjbox@Depth=\dimen262
\adjbox@Totalheight=\dimen263

("C:\Program Files\MiKTeX 2.9\tex\latex\ifoddpage\ifoddpage.sty"
Package: ifoddpage 2016/04/23 v1.1 Conditionals for odd/even page detection
\c@checkoddpage=\count156
))
("C:\Program Files\MiKTeX 2.9\tex\latex\graphics\rotating.sty"
Package: rotating 2016/08/11 v2.16d rotated objects in LaTeX
\c@r@tfl@t=\count157
\rotFPtop=\skip138
\rotFPbot=\skip139
\rot@float@box=\box52
\rot@mess@toks=\toks44
)
("C:\Program Files\MiKTeX 2.9\tex\latex\readarray\readarray.sty"
Package: readarray 2016/11/07\ 2.0\ Routines for inputting 2D and 3D array data
 and recalling it on an element-by-element basis.

("C:\Program Files\MiKTeX 2.9\tex\latex\listofitems\listofitems.sty"
("C:\Program Files\MiKTeX 2.9\tex\generic\listofitems\listofitems.tex"
\loi_nestcnt=\count158
)
Package: listofitems 2016/11/18 v1.3 Grab items in lists using user-specified s
ep char
)
\c@@index=\count159
\c@@plane=\count160
\c@@row=\count161
\c@@col=\count162
\c@use@args=\count163
\c@@record=\count164
\c@arg@index=\count165
\c@break@count=\count166
\c@index@count=\count167
\c@loop@count=\count168
\Arg@toks=\toks45
\@arrayident@toks=\toks46
\rdar@file=\read2

readarray: bounds checking OFF
)
\@RBsgLen=\skip140
\@RBsgWid=\skip141
\@@x=\skip142
\@@y=\skip143
\@RBxA=\skip144
\@RBxB=\skip145
\@RBxC=\skip146
\@RBxD=\skip147
\@RBxS=\skip148
\@RByA=\skip149
\@RByB=\skip150
\@RByC=\skip151
\@RByD=\skip152
\@RBcbxWdtA=\skip153
\@RBcbxWdtB=\skip154
\@RBcbxWdtC=\skip155
\@RBcbxHgtA=\skip156
\@RBcbxHgtB=\skip157
\@RBcbxHgtC=\skip158
\@RBcbxXposA=\skip159
\@RBcbxXposB=\skip160
\@RBcbxXposC=\skip161
\@RBcbxYref=\skip162
\@RBcbxYsep=\skip163
\@RBcbxYsepTotal=\skip164
\@RBcbxYsepShift=\skip165
\@RBcbxHgtTotal=\skip166
\@RBcbxYposA=\skip167
\@RBcbxYposB=\skip168
\@RBcbxYposC=\skip169
\@RBcbxTxtHgtA=\skip170
\@RBcbxTxtHgtB=\skip171
\@RBcbxTxtHgtC=\skip172
\@RBcbxTxtDptA=\skip173
\@RBcbxTxtDptB=\skip174
\@RBcbxTxtDptC=\skip175
\@RBsaveCbxA=\box53
\@RBsaveCbxB=\box54
\@RBsaveCbxC=\box55
\c@@RBneedLF=\count169
\@RBtbxWdt=\skip176
\@RBtbxTxtHgtA=\skip177
\@RBtbxTxtHgtB=\skip178
\@RBtbxTxtHgtC=\skip179
\@RBtbxTxtDptA=\skip180
\@RBtbxTxtDptB=\skip181
\@RBtbxTxtDptC=\skip182
\@RBtbxTxtTotHgtA=\skip183
\@RBtbxTxtTotHgtB=\skip184
\@RBtbxTxtTotHgtC=\skip185
\@RBtbxHgtTotal=\skip186
\@RBtbxYsepAB=\skip187
\@RBtbxYsepBC=\skip188
\@RBsaveTxtA=\box56
\@RBsaveTxtB=\box57
\@RBsaveLenA=\skip189
\@RBsaveLenB=\skip190
\@RBdbxXpos=\skip191
\@RBdbxYref=\skip192
\@RBdbxYpos=\skip193
\@RBdbxWdt=\skip194
\@RBdbxHgtAvail=\skip195
\@RBsaveDbx=\box58
\@RBdbxHgt=\skip196
\@RBdbxDpt=\skip197
\@RBdbxHgtTotal=\skip198
\c@@RBneedDelim=\count170
\c@@cntLine=\count171
\gridPosX=\skip199
\gridPosY=\skip256
) (C:\ProgramData\texmfbosch\tex\latex\bosch\boschfeber.sty
Package: boschfeber 2018/02/13 v4.0.0 Bosch Feber report

Package: boschelements, Stephan Simon, 2001-2018, 2018/02/13 v4.0.0 

("C:\Program Files\MiKTeX 2.9\tex\latex\tools\multicol.sty"
Package: multicol 2017/04/11 v1.8q multicolumn formatting (FMi)
\c@tracingmulticols=\count172
\mult@box=\box59
\multicol@leftmargin=\dimen264
\c@unbalance=\count173
\c@collectmore=\count174
\doublecol@number=\count175
\multicoltolerance=\count176
\multicolpretolerance=\count177
\full@width=\dimen265
\page@free=\dimen266
\premulticols=\dimen267
\postmulticols=\dimen268
\multicolsep=\skip257
\multicolbaselineskip=\skip258
\partial@page=\box60
\last@line=\box61
\maxbalancingoverflow=\dimen269
\mult@rightbox=\box62
\mult@grightbox=\box63
\mult@gfirstbox=\box64
\mult@firstbox=\box65
\@tempa=\box66
\@tempa=\box67
\@tempa=\box68
\@tempa=\box69
\@tempa=\box70
\@tempa=\box71
\@tempa=\box72
\@tempa=\box73
\@tempa=\box74
\@tempa=\box75
\@tempa=\box76
\@tempa=\box77
\@tempa=\box78
\@tempa=\box79
\@tempa=\box80
\@tempa=\box81
\@tempa=\box82
\c@columnbadness=\count178
\c@finalcolumnbadness=\count179
\last@try=\dimen270
\multicolovershoot=\dimen271
\multicolundershoot=\dimen272
\mult@nat@firstbox=\box83
\colbreak@box=\box84
\mc@col@check@num=\count180
)
\@RBfeberTabuW=\skip259
)
("C:\Program Files\MiKTeX 2.9\tex\latex\enumitem\enumitem.sty"
Package: enumitem 2011/09/28 v3.5.2 Customized lists
\labelindent=\skip260
\enit@outerparindent=\dimen273
\enit@toks=\toks47
\enit@inbox=\box85
\enitdp@description=\count181
)
("C:\Program Files\MiKTeX 2.9\tex\latex\amsfonts\amssymb.sty"
Package: amssymb 2013/01/14 v3.01 AMS font symbols
)
("C:\Program Files\MiKTeX 2.9\tex\latex\lastpage\lastpage.sty"
Package: lastpage 2015/03/29 v1.2m Refers to last page's name (HMM; JPG)
){C:/Users/did1tv/AppData/Local/MiKTeX/2.9/pdftex/config/pdftex.map}{C:/Program
Data/texmfbosch/fonts/map/dvips/bosch/boschofficesans.map}
boschcolors: using bright colors
boschcolors: base color is LightGreen
\@saveBoxLogo=\box86
\@saveBoxMyPic=\box87
Package hyperref Info: Option `colorlinks' set `true' on input line 263.
boschformat: using A4 portrait paper format
LaTeX Font Info:    Try loading font information for T1+fbo on input line 455.
(C:\ProgramData\texmfbosch\tex\latex\boschofficesans\t1fbo.fd
File: t1fbo.fd 2016/10/21 Fontinst v1.933 font definitions for T1/fbo.
)
Package typearea Info: These are the values describing the layout:
(typearea)             DIV  = 10
(typearea)             BCOR = 0.0pt
(typearea)             \paperwidth      = 598.14613pt
(typearea)              \textwidth      = 418.70232pt
(typearea)              DIV departure   = -7%
(typearea)              \evensidemargin = 17.45192pt
(typearea)              \oddsidemargin  = 17.45192pt
(typearea)             \paperheight     = 845.90547pt
(typearea)              \textheight     = 595.80026pt
(typearea)              \topmargin      = -25.07945pt
(typearea)              \headheight     = 17.0pt
(typearea)              \headsep        = 20.40001pt
(typearea)              \topskip        = 11.0pt
(typearea)              \footskip       = 47.6pt
(typearea)              \baselineskip   = 13.6pt
(typearea)              on input line 455.

boschcolors: base color is LightGreen
boschcolors: Supergraphic color is Green
\yearcnt=\count182
) (Sim2RealICML2021_IR.aux)
\openout1 = `Sim2RealICML2021_IR.aux'.

LaTeX Font Info:    Checking defaults for OML/cmm/m/it on input line 177.
LaTeX Font Info:    ... okay on input line 177.
LaTeX Font Info:    Checking defaults for T1/cmr/m/n on input line 177.
LaTeX Font Info:    ... okay on input line 177.
LaTeX Font Info:    Checking defaults for OT1/cmr/m/n on input line 177.
LaTeX Font Info:    ... okay on input line 177.
LaTeX Font Info:    Checking defaults for OMS/cmsy/m/n on input line 177.
LaTeX Font Info:    ... okay on input line 177.
LaTeX Font Info:    Checking defaults for OMX/cmex/m/n on input line 177.
LaTeX Font Info:    ... okay on input line 177.
LaTeX Font Info:    Checking defaults for U/cmr/m/n on input line 177.
LaTeX Font Info:    ... okay on input line 177.
LaTeX Font Info:    Checking defaults for PD1/pdf/m/n on input line 177.
LaTeX Font Info:    ... okay on input line 177.
LaTeX Info: Redefining \microtypecontext on input line 177.
Package microtype Info: Generating PDF output.
Package microtype Info: Character protrusion enabled (level 2).
Package microtype Info: Using default protrusion set `alltext'.
Package microtype Info: Automatic font expansion enabled (level 2),
(microtype)             stretch: 20, shrink: 20, step: 1, non-selected.
Package microtype Info: Using default expansion set `basictext'.
Package microtype Info: No adjustment of tracking.
Package microtype Info: No adjustment of interword spacing.
Package microtype Info: No adjustment of character kerning.
Package microtype Info: Loading generic protrusion settings for font family
(microtype)             `fbo' (encoding: T1).
(microtype)             For optimal results, create family-specific settings.
(microtype)             See the microtype manual for details.

("C:\Program Files\MiKTeX 2.9\tex\context\base\supp-pdf.mkii"
[Loading MPS to PDF converter (version 2006.09.02).]
\scratchcounter=\count183
\scratchdimen=\dimen274
\scratchbox=\box88
\nofMPsegments=\count184
\nofMParguments=\count185
\everyMPshowfont=\toks48
\MPscratchCnt=\count186
\MPscratchDim=\dimen275
\MPnumerator=\count187
\makeMPintoPDFobject=\count188
\everyMPtoPDFconversion=\toks49
) ("C:\Program Files\MiKTeX 2.9\tex\latex\oberdiek\epstopdf-base.sty"
Package: epstopdf-base 2016/05/15 v2.6 Base part for package epstopdf

("C:\Program Files\MiKTeX 2.9\tex\latex\oberdiek\grfext.sty"
Package: grfext 2016/05/16 v1.2 Manage graphics extensions (HO)
)
Package epstopdf-base Info: Redefining graphics rule for `.eps' on input line 4
38.
Package grfext Info: Graphics extension search list:
(grfext)             [.pdf,.png,.jpg,.mps,.jpeg,.jbig2,.jb2,.PDF,.PNG,.JPG,.JPE
G,.JBIG2,.JB2,.eps]
(grfext)             \AppendGraphicsExtensions on input line 456.
)
Package caption Info: Begin \AtBeginDocument code.
Package caption Info: float package is loaded.
Package caption Info: hyperref package is loaded.
Package caption Info: rotating package is loaded.
Package caption Info: End \AtBeginDocument code.
\AtBeginShipoutBox=\box89
Package hyperref Info: Link coloring ON on input line 177.

("C:\Program Files\MiKTeX 2.9\tex\latex\hyperref\nameref.sty"
Package: nameref 2016/05/21 v2.44 Cross-referencing by name of section

("C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\gettitlestring.sty"
Package: gettitlestring 2016/05/16 v1.5 Cleanup title references (HO)
)
\c@section@level=\count189
)
LaTeX Info: Redefining \ref on input line 177.
LaTeX Info: Redefining \pageref on input line 177.
LaTeX Info: Redefining \nameref on input line 177.

(Sim2RealICML2021_IR.out) (Sim2RealICML2021_IR.out)
\@outlinefile=\write4
\openout4 = `Sim2RealICML2021_IR.out'.


ABD: EveryShipout initializing macros
Package lastpage Info: Please have a look at the pageslts package at
(lastpage)             https://www.ctan.org/pkg/pageslts
(lastpage)             ! on input line 177.
LaTeX Font Info:    Font shape `T1/fbo/bx/n' in size <10.95> not available
(Font)              Font shape `T1/fbo/b/n' tried instead on input line 182.

("C:\Program Files\MiKTeX 2.9\tex\latex\microtype\mt-cmr.cfg"
File: mt-cmr.cfg 2013/05/19 v2.2 microtype config. file: Computer Modern Roman 
(RS)
)
LaTeX Font Info:    Try loading font information for U+msa on input line 182.

("C:\Program Files\MiKTeX 2.9\tex\latex\amsfonts\umsa.fd"
File: umsa.fd 2013/01/14 v3.01 AMS symbols A
)
("C:\Program Files\MiKTeX 2.9\tex\latex\microtype\mt-msa.cfg"
File: mt-msa.cfg 2006/02/04 v1.1 microtype config. file: AMS symbols (a) (RS)
)
LaTeX Font Info:    Try loading font information for U+msb on input line 182.

("C:\Program Files\MiKTeX 2.9\tex\latex\amsfonts\umsb.fd"
File: umsb.fd 2013/01/14 v3.01 AMS symbols B
)
("C:\Program Files\MiKTeX 2.9\tex\latex\microtype\mt-msb.cfg"
File: mt-msb.cfg 2005/06/01 v1.0 microtype config. file: AMS symbols (b) (RS)
)
<Bosch_4C_S.pdf, id=42, pagebox=cropbox, 426.7905pt x 94.84132pt>
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 229. on input line 
229.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
229.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 229. on input line 
229.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
229.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 229. on input line 
229.
Package pdftex.def Info: Requested size: 82.25021pt x 18.27762pt on input line 
229.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 229. on input line 
229.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
229.
<Bosch-Supergraphic-Green.pdf, id=43, pagebox=cropbox, 1195.0156pt x 506.46013p
t>
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 229. 
on input line 229.
Package pdftex.def Info: Requested size: 478.54616pt x 202.8123pt on input line
 229.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 229. 
on input line 229.
Package pdftex.def Info: Requested size: 28.71924pt x 12.17804pt on input line 
229.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 229. 
on input line 229.
Package pdftex.def Info: Requested size: 478.54616pt x 202.8123pt on input line
 229.

Underfull \hbox (badness 10000) has occurred while \output is active
[]
 []

LaTeX Font Info:    Font shape `T1/fbo/bx/n' in size <8> not available
(Font)              Font shape `T1/fbo/b/n' tried instead on input line 229.

Overfull \hbox (132.40869pt too wide) has occurred while \output is active
[][][][][][][][][][][][][][][][][][][][][][] 
 []


Underfull \hbox (badness 10000) has occurred while \output is active
$[]$ []
 []

[1



 <C:/ProgramData/texmfbosch/tex/generic/images/bosch/CD2016Graphics/Bosch_4C_S.
pdf> <C:/ProgramData/texmfbosch/tex/generic/images/bosch/CD2016Graphics/Bosch-S
upergraphic-Green.pdf>]
LaTeX Font Info:    Font shape `T1/fbo/bx/it' in size <10.95> not available
(Font)              Font shape `T1/fbo/b/it' tried instead on input line 240.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 268. on input line 
268.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
268.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 268. on input line 
268.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
268.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 268. on input line 
268.
Package pdftex.def Info: Requested size: 82.25021pt x 18.27762pt on input line 
268.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 268. on input line 
268.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
268.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 268. 
on input line 268.
Package pdftex.def Info: Requested size: 478.54616pt x 202.8123pt on input line
 268.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 268. 
on input line 268.
Package pdftex.def Info: Requested size: 28.71924pt x 12.17804pt on input line 
268.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 268. 
on input line 268.
Package pdftex.def Info: Requested size: 478.54616pt x 202.8123pt on input line
 268.

Underfull \hbox (badness 10000) has occurred while \output is active
[]
 []


Overfull \hbox (132.40869pt too wide) has occurred while \output is active
[][][][][][][][][][][][][][][][][][][][][][] 
 []


Underfull \hbox (badness 10000) has occurred while \output is active
$[]$ []
 []

[2]
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 292. on input line 
292.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
292.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 292. on input line 
292.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
292.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 292. on input line 
292.
Package pdftex.def Info: Requested size: 82.25021pt x 18.27762pt on input line 
292.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 292. on input line 
292.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
292.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 292. 
on input line 292.
Package pdftex.def Info: Requested size: 478.54616pt x 202.8123pt on input line
 292.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 292. 
on input line 292.
Package pdftex.def Info: Requested size: 28.71924pt x 12.17804pt on input line 
292.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 292. 
on input line 292.
Package pdftex.def Info: Requested size: 478.54616pt x 202.8123pt on input line
 292.

Underfull \hbox (badness 10000) has occurred while \output is active
[]
 []


Overfull \hbox (132.40869pt too wide) has occurred while \output is active
[][][][][][][][][][][][][][][][][][][][][][] 
 []


Underfull \hbox (badness 10000) has occurred while \output is active
$[]$ []
 []

[3]
<s2r_diagram.pdf, id=158, pagebox=cropbox, 483.01051pt x 263.76543pt>
File: s2r_diagram.pdf Graphic file (type pdf)
<use s2r_diagram.pdf>
Package pdftex.def Info: s2r_diagram.pdf  used on input line 326. on input line
 326.
Package pdftex.def Info: Requested size: 382.83838pt x 209.06465pt on input lin
e 326.


LaTeX Warning: Citation `puterman1994markov' on page 4 undefined on input line 
336.

File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 339. on input line 
339.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
339.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 339. on input line 
339.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
339.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 339. on input line 
339.
Package pdftex.def Info: Requested size: 82.25021pt x 18.27762pt on input line 
339.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 339. on input line 
339.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
339.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 339. 
on input line 339.
Package pdftex.def Info: Requested size: 478.54616pt x 202.8123pt on input line
 339.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 339. 
on input line 339.
Package pdftex.def Info: Requested size: 28.71924pt x 12.17804pt on input line 
339.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 339. 
on input line 339.
Package pdftex.def Info: Requested size: 478.54616pt x 202.8123pt on input line
 339.

Underfull \hbox (badness 10000) has occurred while \output is active
[]
 []


Overfull \hbox (132.40869pt too wide) has occurred while \output is active
[][][][][][][][][][][][][][][][][][][][][][] 
 []


Underfull \hbox (badness 10000) has occurred while \output is active
$[]$ []
 []

[4]
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 347. on input line 
347.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
347.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 347. on input line 
347.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
347.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 347. on input line 
347.
Package pdftex.def Info: Requested size: 82.25021pt x 18.27762pt on input line 
347.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 347. on input line 
347.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
347.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 347. 
on input line 347.
Package pdftex.def Info: Requested size: 478.54616pt x 202.8123pt on input line
 347.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 347. 
on input line 347.
Package pdftex.def Info: Requested size: 28.71924pt x 12.17804pt on input line 
347.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 347. 
on input line 347.
Package pdftex.def Info: Requested size: 478.54616pt x 202.8123pt on input line
 347.

Underfull \hbox (badness 10000) has occurred while \output is active
[]
 []


Overfull \hbox (132.40869pt too wide) has occurred while \output is active
[][][][][][][][][][][][][][][][][][][][][][] 
 []


Underfull \hbox (badness 10000) has occurred while \output is active
$[]$ []
 []

[5 <./s2r_diagram.pdf>]
LaTeX Font Info:    Try loading font information for T1+txtt on input line 361.


("C:\Program Files\MiKTeX 2.9\tex\latex\txfonts\t1txtt.fd"
File: t1txtt.fd 2000/12/15 v3.1
)
LaTeX Font Info:    Font shape `T1/txtt/m/it' in size <10.95> not available
(Font)              Font shape `T1/txtt/m/sl' tried instead on input line 361.
Package microtype Info: Loading generic protrusion settings for font family
(microtype)             `txtt' (encoding: T1).
(microtype)             For optimal results, create family-specific settings.
(microtype)             See the microtype manual for details.


AED: lastpage setting LastPage
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 369. on input line 
369.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
369.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 369. on input line 
369.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
369.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 369. on input line 
369.
Package pdftex.def Info: Requested size: 82.25021pt x 18.27762pt on input line 
369.
File: Bosch_4C_S.pdf Graphic file (type pdf)
<use Bosch_4C_S.pdf>
Package pdftex.def Info: Bosch_4C_S.pdf  used on input line 369. on input line 
369.
Package pdftex.def Info: Requested size: 82.25192pt x 18.27762pt on input line 
369.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 369. 
on input line 369.
Package pdftex.def Info: Requested size: 478.54616pt x 202.8123pt on input line
 369.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 369. 
on input line 369.
Package pdftex.def Info: Requested size: 28.71924pt x 12.17804pt on input line 
369.
File: Bosch-Supergraphic-Green.pdf Graphic file (type pdf)
<use Bosch-Supergraphic-Green.pdf>
Package pdftex.def Info: Bosch-Supergraphic-Green.pdf  used on input line 369. 
on input line 369.
Package pdftex.def Info: Requested size: 478.54616pt x 202.8123pt on input line
 369.

Underfull \hbox (badness 10000) has occurred while \output is active
[]
 []


Overfull \hbox (132.40869pt too wide) has occurred while \output is active
[][][][][][][][][][][][][][][][][][][][][][] 
 []


Underfull \hbox (badness 10000) has occurred while \output is active
$[]$ []
 []

[6]
Package atveryend Info: Empty hook `BeforeClearDocument' on input line 369.
Package atveryend Info: Empty hook `AfterLastShipout' on input line 369.
 (Sim2RealICML2021_IR.aux)
Package atveryend Info: Executing hook `AtVeryEndDocument' on input line 369.
Package atveryend Info: Executing hook `AtEndAfterFileList' on input line 369.
Package rerunfilecheck Info: File `Sim2RealICML2021_IR.out' has not changed.
(rerunfilecheck)             Checksum: 91F13A63D35655597B8E8B1140372A6F;855.


LaTeX Warning: There were undefined references.

Package atveryend Info: Empty hook `AtVeryVeryEnd' on input line 369.
 ) 
Here is how much of TeX's memory you used:
 29841 strings out of 493314
 561973 string characters out of 3138865
 827250 words of memory out of 3000000
 32647 multiletter control sequences out of 15000+200000
 40433 words of font info for 183 fonts, out of 3000000 for 9000
 1141 hyphenation exceptions out of 8191
 64i,15n,78p,8832b,913s stack positions out of 5000i,500n,10000p,200000b,50000s
{C:/Program Files/MiKTeX 2.9/fonts/enc/dvips/base/8r.enc}<C:/Program Files/Mi
KTeX 2.9/fonts/type1/public/amsfonts/cm/cmex10.pfb><C:/Program Files/MiKTeX 2.9
/fonts/type1/public/amsfonts/cm/cmmi10.pfb><C:/Program Files/MiKTeX 2.9/fonts/t
ype1/public/amsfonts/cm/cmmi12.pfb><C:/Program Files/MiKTeX 2.9/fonts/type1/pub
lic/amsfonts/cm/cmmi7.pfb><C:/Program Files/MiKTeX 2.9/fonts/type1/public/amsfo
nts/cm/cmmi8.pfb><C:/Program Files/MiKTeX 2.9/fonts/type1/public/amsfonts/cm/cm
r10.pfb><C:/Program Files/MiKTeX 2.9/fonts/type1/public/amsfonts/cm/cmr12.pfb><
C:/Program Files/MiKTeX 2.9/fonts/type1/public/amsfonts/cm/cmr17.pfb><C:/Progra
m Files/MiKTeX 2.9/fonts/type1/public/amsfonts/cm/cmsy10.pfb><C:/Program Files/
MiKTeX 2.9/fonts/type1/public/amsfonts/cm/cmsy8.pfb><C:/ProgramData/texmfbosch/
fonts/type1/bosch/boschofficesans/fbob8a.pfb><C:/ProgramData/texmfbosch/fonts/t
ype1/bosch/boschofficesans/fbobi8a.pfb><C:/ProgramData/texmfbosch/fonts/type1/b
osch/boschofficesans/fbor8a.pfb><C:/ProgramData/texmfbosch/fonts/type1/bosch/bo
schofficesans/fbori8a.pfb><C:/Program Files/MiKTeX 2.9/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb><C:/Program Files/MiKTeX 2.9/fonts/type1/public/txfonts/
t1xtt.pfb>
Output written on Sim2RealICML2021_IR.pdf (6 pages, 489566 bytes).
PDF statistics:
 267 PDF objects out of 1000 (max. 8388607)
 22 named destinations out of 1000 (max. 500000)
 23652 words of extra memory for PDF output out of 24883 (max. 10000000)


